GUI-Libra: Training Native GUI Agents to Reason and Act with Action-aware Supervision and Partially Verifiable RL

Open-source native GUI agents still lag behind closed-source systems on long-horizon navigation tasks. This gap stems from two limitations: a shortage of high-quality, action-aligned reasoning data, and the direct adoption of generic post-training pipelines that overlook the unique challenges of GUI agents. We identify two fundamental issues in these pipelines: (i) standard SFT with CoT reasoning often hurts grounding, and (ii) step-wise RLVR-tyle training faces partial verifiability, where multiple actions can be correct but only a single demonstrated action is used for verification. This makes offline step-wise metrics weak predictors of online task success. In this work, we present GUI-Libra, a tailored training recipe that addresses these challenges. First, to mitigate the scarcity of action-aligned reasoning data, we introduce a data construction and filtering pipeline and release a curated 81K GUI reasoning dataset. Second, to reconcile reasoning with grounding, we propose action-aware SFT that mixes reasoning-then-action and direct-action data and reweights tokens to emphasize action and grounding. Third, to stabilize RL under partial verifiability, we identify the overlooked importance of KL regularization in RLVR and show that a KL trust region is critical for improving offline-to-online predictability; we further introduce success-adaptive scaling to downweight unreliable negative gradients. Across diverse web and mobile benchmarks, GUI-Libra consistently improves both step-wise accuracy and end-to-end task completion. Our results suggest that carefully designed post-training and data curation can unlock significantly stronger task-solving capabilities without costly online data collection. We release our dataset, code, and models to facilitate further research on data-efficient post-training for reasoning-capable GUI agents.

==> sections/additional_metrics_old.tex <==
\begin{table}[]
\centering
\caption{Grounding Accuracy on AndroidControl-v2.}
\label{tab:AC_grounding_accuracy}
\resizebox{0.75\linewidth}{!}{
\begin{tabular}{lllll}
\toprule
 & \multicolumn{2}{c}{\textbf{High Level}} 
 & \multicolumn{2}{c}{\textbf{Low Level}} \\
\textbf{Model}
 & Pass@1 & Pass@4 
 & Pass@1 & Pass@4  \\

\midrule
\multicolumn{5}{c}{\textbf{Proprietary Models with SeeAct-V Framework}}\\
\midrule

GPT-4o + UGround-v1-7B  & 58.7 & 67.3
& 83.4 & 88.3 \\

GPT-4.1 + UGround-v1-7B  & 60.5 & 64.6
& 83.0 & 86.1 \\

GPT-5-mini + UGround-v1-7B  & 61.9 & 66.8
& 83.9 & 87.9 \\

GPT-5 + UGround-v1-7B  & \underline{74.4} & \textbf{82.1}
& \underline{93.7} & 94.6 \\

\midrule
\multicolumn{5}{c}{\textbf{Open-source Native Models}}\\
\midrule

 GUI-R1-3B & 53.4 & 66.4
& 81.2 & 87.0 \\

  GUI-R1-7B  & 58.3 & 72.2
& 87.9 & 87.9 \\
 

Aguvis-7B
 & 67.3 & 78.0 
 & 85.7 & 87.0  \\

 UI-TARS-1.5-7B
 & 57.9 & 71.3
 & 78.5 & 88.8 \\

 
GLM-4.1V-9B-Thinking
 & 44.0 & 55.6 
 & 68.2 & 75.8  \\


Qwen2.5-VL-32B
 & 49.0 & 66.6 
 & 78.4 & 85.4 \\

Qwen2.5-VL-72B
 & 56.5 & 72.9 
 & 82.9 & 90.2 \\

 Qwen3-VL-32B  & 70.9 & 79.4
& 91.9 & 93.3 \\


\midrule
Qwen2.5-VL-3B (Baseline)
 & 42.2 & 46.6 
 & 78.0 & 80.7\\

% \rowcolor{beijingblue}
% \textbf{GUI-Libra-3B old (Ours)}
%  & 64.1 {\scriptsize (+21.9)}
%  & 74.0 {\scriptsize (+27.4)}
%  & 88.3 {\scriptsize (+10.3)}
%  & 92.8 {\scriptsize (+12.1)} \\

\rowcolor{beijingblue}
\textbf{GUI-Libra-3B (Ours)}
 & 68.2 & 77.1
  & 89.2 & 91.5 \\

Qwen2.5-VL-7B (Baseline)
 & 60.5 & 69.5 
 & 82.5 & 88.3  \\

% \rowcolor{beijingblue}
% \textbf{GUI-Libra-7B old (Ours)}
%  & \underline{74.4} {\scriptsize (+13.9)}
%  & 79.4 {\scriptsize (+9.9)}
%  & 92.4 {\scriptsize (+9.9)}
%  & \underline{95.5} {\scriptsize (+7.2)} \\

 \rowcolor{beijingblue}
\textbf{GUI-Libra-7B (Ours)}
 & 71.8 & 78.0
  & 91.5 & 93.7 \\

 Qwen3-VL-4B (Baseline) & 65.9 & 76.7
 & 90.6 & 93.3 \\

% \rowcolor{beijingblue}
% \textbf{GUI-Libra-4B (Ours)}  & 73.1 {\scriptsize (+7.2)}
%  & \underline{80.7} {\scriptsize (+4.0)}
%  & 90.1 {\scriptsize (-0.5)}
%  & 93.3 {\scriptsize (+0.0)} \\

\rowcolor{beijingblue}
\textbf{GUI-Libra-4B  (Ours)} 
 & 74.0 & \underline{81.6}
 & 91.0 & \underline{95.1} \\

 Qwen3-VL-8B (Baseline)   & 67.7 & 79.8
 & 93.3 & \underline{95.1} \\

% \rowcolor{beijingblue}
% \textbf{GUI-Libra-8B (Ours)}  & \textbf{80.3} {\scriptsize (+12.6)}
%  & \textbf{82.1} {\scriptsize (+2.2)}
%  & \textbf{95.5} {\scriptsize (+2.3)}
%  & \textbf{96.0} {\scriptsize (+0.9)} \\

\rowcolor{beijingblue}
\textbf{GUI-Libra-8B (Ours)} 
  & \textbf{76.2} & \underline{81.6}
 & \textbf{95.5} & \textbf{96.4} \\


\bottomrule
\end{tabular}}
\end{table}



\begin{table}[]
\centering
\caption{Type Accuracy on AndroidControl-v2.}
\label{tab:ac_type_accuracy}
\resizebox{0.75\linewidth}{!}{
\begin{tabular}{lllll}
\toprule
 & \multicolumn{2}{c}{\textbf{High Level}} 
 & \multicolumn{2}{c}{\textbf{Low Level}} \\
\textbf{Model}
 & Pass@1 & Pass@4 
 & Pass@1 & Pass@4  \\
\midrule
\multicolumn{5}{c}{\textbf{Proprietary Models with SeeAct-V Framework}}\\
\midrule

GPT-4o + UGround-v1-7B & 73.9 & 82.7
& 89.2 & 93.7 \\

GPT-4.1 + UGround-v1-7B & 72.9 & 78.9
& 89.5 & 93.0 \\

GPT-5-mini + UGround-v1-7B  & 70.9 & 77.4
& 89.7 & 93.5 \\

GPT-5 + UGround-v1-7B  & \textbf{74.1} & 78.9
& 88.4 & 91.5 \\

\midrule
\multicolumn{5}{c}{\textbf{Open-source Native Models}}\\
\midrule

GUI-R1-3B & 63.1 & 76.4
& 71.1 & 90.2 \\

GUI-R1-7B  & 61.8 & 76.1
& 76.1 & 89.2 \\

Aguvis-7B  & 58.0 & 59.8 
 & 60.6 & 62.1 \\

 UI-TARS-1.5-7B
 & 69.4 & \textbf{87.4} 
 & 70.9 & 91.0 \\

GLM-4.1V-9B-Thinking
 & 65.8 & 74.1 
 & 89.2 & 92.5 \\

Qwen2.5-VL-32B  & 67.3 & 78.1 
 & 85.7 & 89.7 \\

Qwen2.5-VL-72B  & 72.9 &\underline{86.9}
 & 89.5 & \textbf{96.2}\\

Qwen3-VL-32B  & \underline{73.6} & 81.2
& 90.2 & 92.2 \\

\midrule
Qwen2.5-VL-3B (Baseline)  & 53.0 & 77.4 
 & 80.2 & 90.0 \\

% \rowcolor{beijingblue}
% \textbf{GUI-Libra-3B old (Ours)}   
%  & 65.8 {\scriptsize (+12.8)}
%  & 74.1 {\scriptsize (-3.3)}
%  & 88.4 {\scriptsize (+8.2)}
%  & 92.2 {\scriptsize (+2.2)} \\

\rowcolor{beijingblue}
\textbf{GUI-Libra-3B  (Ours)}  
 & 70.4 & 78.1
 & 89.5 & 93.7 \\
 
Qwen2.5-VL-7B (Baseline) & 62.8 & 77.4 
 & 78.6 & 91.7  \\

% \rowcolor{beijingblue}
% \textbf{GUI-Libra-7B old (Ours)}
%  & 72.4 {\scriptsize (+9.6)}
%  & 77.6 {\scriptsize (+0.2)}
%  & 89.5 {\scriptsize (+10.9)}
%  & 93.7 {\scriptsize (+2.0)} \\

\rowcolor{beijingblue}
\textbf{GUI-Libra-7B  (Ours)}
 & 72.9 & 78.6
 & 88.9 & 91.2 \\

Qwen3-VL-4B (Baseline)  & 63.6 & 78.4
 & 86.4 & 88.7 \\

% \rowcolor{beijingblue}
% \textbf{GUI-Libra-4B old (Ours)}
%  & 71.6 {\scriptsize (+8.0)}
%  & 78.1 {\scriptsize (-0.2)}
%  & \underline{94.0} {\scriptsize (+7.5)}
%  & \textbf{96.5} {\scriptsize (+7.8)} \\

\rowcolor{beijingblue}
\textbf{GUI-Libra-4B  (Ours)}
 & 72.6 & 76.1
 & \underline{92.5} & 95.0 \\

Qwen3-VL-8B (Baseline)   & 68.8 & 77.6
 & 82.4 & 86.9 \\

% \rowcolor{beijingblue}
% \textbf{GUI-Libra-8B old (Ours)}  & \textbf{75.1} {\scriptsize (+6.3)}
%  & 79.9 {\scriptsize (+2.3)}
%  & \textbf{95.0} {\scriptsize (+12.6)}
%  & \underline{96.2} {\scriptsize (+9.3)} \\

\rowcolor{beijingblue}
\textbf{GUI-Libra-8B  (Ours)} 
 & \textbf{74.1} & 78.9
 & \textbf{93.7} & \underline{95.5} \\
 
\bottomrule
\end{tabular}}
\end{table}






\begin{table}[t]
\centering
\caption{Grounding accuracy (\%) on Multimodal-Mind2Web-v2.}
\label{tab:mind2web_grounding}
\resizebox{\linewidth}{!}{
\begin{tabular}{lllllllll}
\toprule
& \multicolumn{2}{c}{Cross-Task} 
& \multicolumn{2}{c}{Cross-Website} 
& \multicolumn{2}{c}{Cross-Domain} 
& \multicolumn{2}{c}{Average} \\
\textbf{Model}
& Pass@1 & Pass@4  & Pass@1 & Pass@4   & Pass@1 & Pass@4   & Pass@1 & Pass@4 \\
\midrule
\multicolumn{9}{c}{\textbf{Proprietary Models with SeeAct-V Framework}}\\
\midrule


GPT-4o + UGround-v1-7B & 42.0 & 44.0 & 40.6 & 42.9 & 44.9 & 47.2 & 42.5 & 44.7 \\

GPT-4.1 + UGround-v1-7B   & 47.4 & 49.3
 & 43.5 & 45.5
 & 48.7 & 51.4
 & 46.5 & 48.7 \\

GPT-5-mini + UGround-v1-7B  & 52.5 & 53.1 & 50.7 & 51.6 & 53.6 & 54.3 & 52.3 & 53.0 \\

GPT-5 + UGround-v1-7B   & 55.3 & 56.6
 & 53.1 & 53.4
 & 55.8 & 57.3
 & 54.7 & 55.8 \\

\midrule
\multicolumn{9}{c}{\textbf{Open-source Native Models}}\\
\midrule


GUI-R1-3B 
& 29.1 & 44.6 & 27.2 & 45.5 & 29.1 & 44.9 & 28.5 & 45.0 \\

GUI-R1-7B  & 43.8 & 56.8 & 40.6 & 54.9 & 45.7 & 56.3 & 43.4 & 56.0 \\


Aguvis-7B
& 40.5 & 53.5
& 34.9 & 47.4
& 38.8 & 48.8
& 38.1 & 49.9 \\

UI-TARS-1.5-7B
& 46.2 & 59.0
& 42.2 & 57.6
& 46.4 & 60.2
& 45.0 & 58.9 \\

GLM-4.1V-9B-Thinking
& 36.8 & 42.8
& 34.2 & 39.7
& 36.9 & 44.1
& 36.0 & 42.2 \\

 
Qwen2.5-VL-32B & 53.0 & 61.8 & 50.9 & \underline{61.6} & 52.6 & 62.9 & 52.2 & 62.1 \\

Qwen2.5-VL-72B
& 55.7 & \textbf{65.0} & 53.7 & 61.5 & 56.3 & \textbf{64.4} & 55.2 & \textbf{63.6} \\

Qwen3-VL-32B 
& 55.9 & 62.4 & 52.7 & \textbf{61.7} & \underline{56.7} & \underline{63.9} & 55.1 & \underline{62.7} \\

 \midrule
Qwen2.5-VL-3B (Baseline)
& 37.9 & 40.1 & 35.6 & 38.6 & 38.8 & 43.2 & 37.4 & 40.6 \\

 
% \rowcolor{beijingblue}
% \textbf{GUI-Libra-3B old (Ours)}
% & 50.6 
% & 56.9 
% & 49.0 
% & 57.0 
% & 51.1 
% & 58.7 
% & 50.2 {\scriptsize (+12.8)}
% & 57.5 {\scriptsize (+16.9)} \\

\rowcolor{beijingblue}
\textbf{GUI-Libra-3B (Ours)}
 & 50.1 & 57.8
 & 50.7 & 58.6
 & 51.6 & 58.5
 & 50.8 & 58.3 \\

 
Qwen2.5-VL-7B (Baseline)
& 44.1 & 54.0 & 45.5 & 54.2 & 46.2 & 57.4 & 45.3 & 55.2 \\


% \rowcolor{beijingblue}
% \textbf{GUI-Libra-7B old (Ours)}
% & 54.9 
% & 61.1 
% & 53.9 
% & 61.0 
% & 55.2 
% & 61.5 
% & 54.7 {\scriptsize (+9.4)}
% & 61.2 {\scriptsize (+6.0)} \\

\rowcolor{beijingblue}
\textbf{GUI-Libra-7B (Ours)}
 & 53.5 & 59.8
 & 54.2 & 60.4
 & 53.6 & 60.7
 & 53.7 & 60.3 \\


Qwen3-VL-4B (Baseline) 
 & 49.9 & 59.6 & 47.9 & 58.2 & 49.9 & 57.5 & 49.2 & 58.4 \\


% \rowcolor{beijingblue}
% \textbf{GUI-Libra-4B old (Ours)}
% & 54.4 & 61.5
%  & \underline{55.3} & 61.2
%  & 56.1 & 61.6
%  & \underline{55.2} {\scriptsize (+6.0)} & 61.4  {\scriptsize (+3.0)}\\

\rowcolor{beijingblue}
\textbf{GUI-Libra-4B  (Ours)}
  & \underline{57.2} & 61.7
 & \underline{56.2} & 61.4
 & \underline{56.7} & 62.1
 &\underline{56.7} & 61.7 \\
 

Qwen3-VL-8B (Baseline)
& 52.6 & 60.0 & 49.6 & 59.3 & 52.4 & 59.3 & 51.5 & 59.5 \\

% \rowcolor{beijingblue}
% \textbf{GUI-Libra-8B old (Ours)}
% & \textbf{58.4} 
% & 62.2 
% & \textbf{55.6} 
% & 60.7 
% & \textbf{57.8} 
% & 61.5 
% & \textbf{57.3} {\scriptsize (+5.8)}
% & 61.4 {\scriptsize (+1.9)} \\

\rowcolor{beijingblue}
\textbf{GUI-Libra-8B (Ours)}
 & \textbf{58.6} & \underline{62.6}
 & \textbf{56.5} & 61.2
 & \textbf{58.2} & 62.5
 & \textbf{57.8} & 62.1 \\

\bottomrule
\end{tabular}}
\end{table}



\begin{table}[t]
\centering
\caption{Operation F1 score on Multimodal-Mind2Web-v2.}
\label{tab:mind2web_operation_f1}
\resizebox{\linewidth}{!}{
\begin{tabular}{lllllllll}
\toprule
& \multicolumn{2}{c}{Cross-Task} 
& \multicolumn{2}{c}{Cross-Website} 
& \multicolumn{2}{c}{Cross-Domain} 
& \multicolumn{2}{c}{Average} \\
\textbf{Model}
& Best@1 & Best@4  & Best@1 & Best@4   & Best@1 & Best@4  & Best@1 & Best@4 \\
\midrule
\multicolumn{9}{c}{\textbf{Proprietary Models with SeeAct-V Framework}}\\
\midrule


GPT-4o + UGround-v1-7B  & 70.1 & 78.9 & 70.9 & 79.6 & 67.7 & 75.7 & 69.6 & 78.1 \\

GPT-4.1 + UGround-v1-7B   & 72.7 & 81.6
 & 71.1 & 81.0
 & 71.1 & 79.4
 & 71.6 & 80.7 \\

GPT-5-mini + UGround-v1-7B  & 80.7 & 88.8 & 77.3 & 86.8 & 77.9 & 85.3 & 78.6 & 87.0 \\

GPT-5 + UGround-v1-7B   & 79.7 & 89.2
 & 79.6 & 88.9
 & 79.1 & 88.2
 & 79.5 & 88.8 \\ 

\midrule
\multicolumn{9}{c}{\textbf{Open-source Native Models}}\\
\midrule

GUI-R1-3B  & 79.5 & 87.9 & 75.4 & 85.3 & 79.6 & 89.4 & 78.1 & 87.5 \\

GUI-R1-7B  & 78.9 & 89.6 & 75.2 & 88.5 & 79.8 & 90.7 & 78.0 & 89.6 \\

Aguvis-7B
& 84.4 & 91.1
& 80.7 & 87.9
& 83.3 & 91.5
& 82.8 & 90.2 \\

UI-TARS-1.5-7B
& 81.2 & 85.3
& 78.5 & 81.6
& 81.1 & 85.0
& 80.3 & 84.0 \\

GLM-4.1V-9B-Thinking
& 73.6 & 82.0
& 69.2 & 80.0
& 73.7 & 81.6
& 72.2 & 81.2 \\


Qwen2.5-VL-32B
& 84.2 & \underline{92.6} & 81.9 & \textbf{92.0} & 82.6 & \textbf{93.0} & 82.9 & \underline{92.5} \\

Qwen2.5-VL-72B
& \underline{85.2} & \textbf{93.5} & 83.3 & \underline{91.5} & 84.3 & \textbf{93.0} & \underline{84.3} & \textbf{92.7} \\


Qwen3-VL-32B 
& 83.9 & 91.6 & 81.3 & 89.9 & 83.7 & \underline{92.2} & 83.0 & 91.2 \\

 \midrule
Qwen2.5-VL-3B (Baseline)
& 59.3 & 86.5 & 51.6 & 83.0 & 64.7 & 88.3 & 58.5 & 85.9 \\

% \rowcolor{beijingblue}
% \textbf{GUI-Libra-3B old (Ours)}
% & 84.4
% & 88.4
% & 81.1
% & 85.4
% & \textbf{86.5}
% & 90.7
% & 84.0 {\scriptsize (+25.5)}
% & 88.2 {\scriptsize (+2.3)} \\


\rowcolor{beijingblue}
\textbf{GUI-Libra-3B (Ours)}
 & 84.6 & 88.0
 & 80.8 & 85.2
 & \textbf{86.4} & 89.2
 & 83.9 & 87.5 \\

Qwen2.5-VL-7B (Baseline)
 & 68.1 & 90.9 & 66.7 & 90.4 & 73.3 & 91.6 & 69.4 & 91.0 \\


% \rowcolor{beijingblue}
% \textbf{GUI-Libra-7B old (Ours)}
% & \underline{84.6}
% & 88.1
% & \textbf{84.0}
% & 87.5
% & \underline{85.7}
% & 89.6
% & \textbf{84.8} {\scriptsize (+15.4)}
% & 88.4 {\scriptsize (-2.6)} \\

\rowcolor{beijingblue}
\textbf{GUI-Libra-7B  (Ours)}
 & \underline{85.2} & 88.1
 & \textbf{84.3} & 88.2
 & \underline{85.9} & 89.4
 & \textbf{85.1} & 88.6 \\


Qwen3-VL-4B (Baseline) 
& 81.6 & 88.9 & 78.9 & 88.2 & 79.5 & 89.9 & 80.0 & 89.0 \\

% \rowcolor{beijingblue}
% \textbf{GUI-Libra-4B old (Ours)} 
%  & 84.0 & 88.6
%  & 82.4 & 87.1
%  & 82.2 & 87.0
%  & 82.9 {\scriptsize (+2.9)} & 87.6 {\scriptsize (-1.1)} \\

\rowcolor{beijingblue}
\textbf{GUI-Libra-4B (Ours)} 
  & 85.0 & 88.9
 & \underline{83.6} & 88.2
 & 82.8 & 88.1
 & 83.8 & 88.4 \\
 


Qwen3-VL-8B (Baseline) 
 & 83.2 & 91.2 & 80.0 & 89.0 & 82.7 & 90.2 & 82.0 & 90.1 \\

% \rowcolor{beijingblue}
% \textbf{GUI-Libra-8B old (Ours)}
% & 84.5
% & 88.5
% & \underline{83.7}
% & 88.3
% & 83.8
% & 88.1
% & 84.0 {\scriptsize (+2.0)}
% & 88.3 {\scriptsize (-1.8)} \\

\rowcolor{beijingblue}
\textbf{GUI-Libra-8B  (Ours)}
 & \textbf{85.5} & 88.1
 & 81.8 & 86.9
 & 84.4 & 87.0
 & 83.9 & 87.3 \\

\bottomrule
\end{tabular}}
\end{table}
